Compiler Optimization: A Case for the Transformation Tool Contest

An optimizing compiler consists of a front end parsing a textual programming language into an intermediate representation (IR), a middle end performing optimizations on the IR, and a back end lowering the IR to a target representation (TR) built of operations supported by the target hardware. In modern compiler construction graph-based IRs are employed. Optimization and lowering tasks can then be implemented with graph transformation rules. This case provides two compiler tasks to evaluate the participating tools regarding performance.

==> eptcsdata.tex <==
\providecommand{\firstpage}{6}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.2}{10.4204/EPTCS.74.2}}
\pdfoutput=1

